Chrono-chemodynamical analysis of the globular cluster NGC 6355: Looking for the fundamental bricks of the Bulge

The information on Galactic assembly time is imprinted on the chemodynamics of globular clusters. This makes them important probes that help us to understand the formation and evolution of the Milky Way. Discerning between in-situ and ex-situ origin of these objects is difficult when we study the Galactic bulge, which is the most complex and mixed component of the Milky Way. To investigate the early evolution of the Galactic bulge, we analysed the globular cluster NGC 6355. We derived chemical abundances and kinematic and dynamic properties by gathering information from high-resolution spectroscopy with FLAMES-UVES, photometry with the Hubble Space Telescope, and Galactic dynamic calculations applied to the globular cluster NGC 6355. We derive an age of $13.2\pm1.1$ Gyr and a metallicity of [Fe/H]$=-1.39\pm0.08$ for NGC 6355, with $\alpha$-enhancement of [$\alpha$/Fe]$=+0.37\pm0.11$. The abundance pattern of the globular cluster is compatible with bulge field RR Lyrae stars and in-situ well-studied globular clusters. The orbital parameters suggest that the cluster is currently confined within the bulge volume when we consider a heliocentric distance of $8.54\pm0.19$ kpc and an extinction coefficient of $R_V = 2.84\pm0.02$. NGC 6355 is highly likely to come from the main bulge progenitor. {Nevertheless, it still} has a low probability of being formed from an accreted event because its age is uncertain and because of the combined [Mg/Mn] [Al/Fe] abundance. Its relatively low metallicity with respect to old and moderately metal-poor inner Galaxy clusters may suggest a low-metallicity floor for globular clusters that formed in-situ in the early Galactic bulge.

==> feh_ews.tex <==
\onecolumn
\begin{longtable}{lcccccccc}
\caption{Equivalent widths for \ion{Fe}{I} and \ion{Fe}{II} lines.  }            
\label{tab:fe}\\      

\hline
\noalign{\smallskip}
\multirow{2}{*}{Ion} & $\lambda$ & $\chi_{ex}$  & \multirow{2}{*}{log$gf$} &     star 1539   &    star 1363   &     star 1176  &  star 133 \\ 
                     &  [\AA]  &  [eV]        &                          & \multicolumn{4}{c}{[m \AA]}\\ 
\hline\hline \endfirsthead
\multicolumn{8}{c}%
{{\bfseries \tablename\ \thetable{} -- continued}} \\ \hline
Ion & $\lambda$ & $\chi_{ex}$  & log$gf$ &     star 1539   &    star 1363   &     star 1176  &  star 133\\ 
%    &  [$\AA$]  &  [eV]        &         & [m$\AA$] & [m$\AA$] & [m$\AA$] & [m$\AA$] & [m$\AA$] & [m$\AA$] \\ 
\hline\hline \endhead

   \ion{Fe}{II} & $5991.38$ & $3.10$ & $-3.65$  &   ---    & $ 21.1$ & $ 33.4$ & $ 17.0$ \\ 
   \ion{Fe}{II} & $6084.11$ & $3.20$ & $-3.97$  &   ---    & $ 16.8$ & $ 13.2$ & $ 11.8$ \\ 
   \ion{Fe}{II} & $6149.25$ & $3.80$ & $-2.69$  &   ---    & $ 62.4$ & $ 28.1$ & $ 17.5$ \\ 
   \ion{Fe}{II} & $6247.56$ & $3.80$ & $-2.30$  &  $ 41.6$ &  ---    & $ 47.1$ & $ 29.9$ \\ 
   \ion{Fe}{II} & $6416.93$ & $3.80$ & $-2.64$  &  $ 29.7$ & $ 34.6$ & $ 25.5$ & $ 18.1$ \\ 
   \ion{Fe}{II} & $6432.68$ & $2.80$ & $-3.57$  &  $ 42.2$ & $ 42.4$ & $ 40.2$ & $ 33.1$ \\ 
   \ion{Fe}{II} & $6456.39$ & $3.90$ & $-2.31$  &   ---    & $ 48.2$ & $ 61.7$ & $ 40.8$ \\ 
   \ion{Fe}{II} & $6516.08$ & $2.80$ & $-3.31$  &  $ 53.8$ & $ 17.1$ & $ 47.0$ & $ 42.7$ \\ 
   \hline
    \ion{Fe}{I} & $5905.67$ & $4.60$ & $-0.73$  &   ---    & $ 30.3$ &  ---    & $ 27.2$ \\ 
    \ion{Fe}{I} & $5916.25$ & $2.40$ & $-2.97$  &  $ 87.1$ &  ---    & $ 55.6$ &  ---    \\ 
    \ion{Fe}{I} & $5927.79$ & $4.60$ & $-1.09$  &   ---    & $ 23.7$ & $ 17.1$ & $ 19.3$ \\ 
    \ion{Fe}{I} & $5929.67$ & $4.50$ & $-1.41$  &  $ 23.9$ & $ 17.7$ & $ 14.4$ & $ 16.0$ \\ 
    \ion{Fe}{I} & $5930.18$ & $4.60$ & $-0.23$  &  $ 66.3$ & $ 62.6$ & $ 46.7$ & $ 49.9$ \\ 
    \ion{Fe}{I} & $5934.65$ & $3.90$ & $-1.17$  &  $ 70.3$ &  ---    & $ 49.0$ & $ 54.2$ \\ 
    \ion{Fe}{I} & $5952.73$ & $3.90$ & $-1.44$  &  $ 50.9$ & $ 49.2$ & $ 38.9$ & $ 43.3$ \\ 
    \ion{Fe}{I} & $5956.69$ & $0.80$ & $-4.60$  &  $119.8$ &  ---    & $ 78.4$ &  ---    \\ 
    \ion{Fe}{I} & $5975.35$ & $4.80$ & $-0.69$  &  $ 33.6$ & $ 35.7$ & $ 23.6$ &  ---    \\ 
    \ion{Fe}{I} & $5983.69$ & $4.50$ & $-1.47$  &   ---    & $ 44.4$ & $ 34.0$ &  ---    \\ 
    \ion{Fe}{I} & $5987.06$ & $4.80$ & $-0.43$  &  $ 39.7$ &  ---    & $ 25.3$ &  ---    \\ 
    \ion{Fe}{I} & $6003.01$ & $3.80$ & $-1.12$  &  $ 74.9$ & $ 74.5$ & $ 54.2$ & $ 65.3$ \\ 
    \ion{Fe}{I} & $6005.54$ & $2.50$ & $-3.61$  &  $ 37.8$ & $ 41.6$ & $ 19.2$ & $ 24.9$ \\ 
    \ion{Fe}{I} & $6008.56$ & $3.80$ & $-0.99$  &  $ 84.3$ &  ---    & $ 60.1$ & $ 67.0$ \\ 
    \ion{Fe}{I} & $6020.17$ & $4.60$ & $-0.27$  &  $ 73.3$ &  ---    & $ 50.0$ & $ 54.5$ \\ 
    \ion{Fe}{I} & $6024.05$ & $4.50$ & $-0.12$  &  $ 82.2$ & $ 85.0$ & $ 67.4$ & $ 72.0$ \\ 
    \ion{Fe}{I} & $6027.06$ & $4.00$ & $-1.09$  &  $ 55.7$ & $ 57.8$ & $ 34.0$ & $ 38.6$ \\ 
    \ion{Fe}{I} & $6054.08$ & $4.30$ & $-2.31$  &   ---    &  ---    &  ---    &  ---    \\ 
    \ion{Fe}{I} & $6065.48$ & $2.60$ & $-1.53$  &  $148.7$ &  ---    & $124.5$ &  ---    \\ 
    \ion{Fe}{I} & $6078.49$ & $4.80$ & $-0.32$  &  $ 43.5$ & $ 45.5$ & $ 26.9$ & $ 37.8$ \\ 
    \ion{Fe}{I} & $6079.01$ & $4.60$ & $-1.12$  &  $ 21.2$ & $ 23.2$ & $ 13.6$ & $ 17.0$ \\ 
    \ion{Fe}{I} & $6082.71$ & $2.20$ & $-3.57$  &  $ 67.4$ & $ 69.1$ & $ 33.1$ & $ 50.0$ \\ 
    \ion{Fe}{I} & $6093.64$ & $4.60$ & $-1.50$  &  $ 20.3$ & $ 14.6$ & $ 20.1$ & $ 12.8$ \\ 
    \ion{Fe}{I} & $6137.70$ & $2.50$ & $-1.40$  &   ---    &  ---    & $137.6$ &  ---    \\ 
    \ion{Fe}{I} & $6151.62$ & $2.10$ & $-3.30$  &  $ 82.6$ &  ---    & $ 53.7$ & $ 72.7$ \\ 
%    \ion{Fe}{I} & $6159.38$ & $4.60$ & $-1.97$  &   ---    &  ---    &  ---    &  ---    \\ 
    \ion{Fe}{I} & $6165.36$ & $4.10$ & $-1.47$  &  $ 32.4$ & $ 30.1$ & $ 16.6$ & $ 17.6$ \\ 
    \ion{Fe}{I} & $6180.21$ & $2.70$ & $-2.59$  &  $ 82.4$ & $ 84.8$ & $ 49.6$ & $ 64.2$ \\ 
    \ion{Fe}{I} & $6187.99$ & $3.90$ & $-1.72$  &  $ 40.0$ & $ 37.3$ & $ 22.4$ & $ 31.8$ \\ 
    \ion{Fe}{I} & $6213.44$ & $2.20$ & $-2.48$  &  $122.4$ &  ---    & $ 96.4$ &  ---    \\ 
    \ion{Fe}{I} & $6219.29$ & $2.20$ & $-2.43$  &  $131.7$ &  ---    & $109.2$ &  ---    \\ 
    \ion{Fe}{I} & $6220.78$ & $3.80$ & $-2.46$  &  $ 10.3$ &  ---    &  ---    &  ---    \\ 
    \ion{Fe}{I} & $6226.73$ & $3.80$ & $-2.22$  &  $ 17.5$ & $ 23.1$ & $ 13.8$ & $ 16.1$ \\ 
    \ion{Fe}{I} & $6252.57$ & $2.40$ & $-1.69$  &   ---    &  ---    & $134.3$ &  ---    \\ 
    \ion{Fe}{I} & $6254.25$ & $2.20$ & $-2.44$  &  $133.7$ &  ---    & $114.8$ &  ---    \\ 
    \ion{Fe}{I} & $6265.14$ & $2.10$ & $-2.55$  &  $128.2$ &  ---    & $110.6$ &  ---    \\ 
    \ion{Fe}{I} & $6270.23$ & $2.80$ & $-2.46$  &  $ 71.7$ & $ 76.1$ & $ 42.6$ & $ 58.0$ \\ 
    \ion{Fe}{I} & $6271.28$ & $3.30$ & $-2.70$  &  $ 27.4$ & $ 27.3$ & $ 15.2$ & $ 16.9$ \\ 
    \ion{Fe}{I} & $6301.51$ & $3.60$ & $-0.72$  &  $104.0$ &  ---    & $ 86.7$ &  ---    \\ 
    \ion{Fe}{I} & $6311.50$ & $2.80$ & $-3.14$  &  $ 43.6$ & $ 42.7$ & $ 23.3$ & $ 28.9$ \\ 
    \ion{Fe}{I} & $6315.31$ & $4.10$ & $-1.23$  &  $ 45.3$ & $ 41.9$ & $ 28.3$ &  ---    \\ 
    \ion{Fe}{I} & $6315.81$ & $4.00$ & $-1.71$  &  $ 29.2$ & $ 28.7$ & $ 10.3$ & $ 18.2$ \\ 
    \ion{Fe}{I} & $6335.34$ & $2.20$ & $-2.18$  &  $142.7$ &  ---    & $122.2$ &  ---    \\ 
    \ion{Fe}{I} & $6344.16$ & $2.40$ & $-2.92$  &  $ 91.2$ &  ---    & $ 62.8$ & $ 72.9$ \\ 
    \ion{Fe}{I} & $6380.75$ & $4.10$ & $-1.38$  &  $ 42.2$ & $ 35.9$ & $ 26.3$ & $ 33.5$ \\ 
    \ion{Fe}{I} & $6392.54$ & $2.20$ & $-4.03$  &  $ 36.9$ & $ 37.5$ &  ---    &  ---    \\ 
    \ion{Fe}{I} & $6393.61$ & $2.40$ & $-1.43$  &   ---    &  ---    & $140.8$ &  ---    \\ 
    \ion{Fe}{I} & $6411.66$ & $3.60$ & $-0.60$  &  $115.8$ &  ---    & $ 98.5$ & $101.7$ \\ 
    \ion{Fe}{I} & $6419.94$ & $4.70$ & $-0.24$  &  $ 57.5$ & $ 55.9$ & $ 40.6$ & $ 45.1$ \\ 
    \ion{Fe}{I} & $6421.35$ & $2.20$ & $-2.03$  &   ---    &  ---    & $132.5$ &  ---    \\ 
    \ion{Fe}{I} & $6430.86$ & $2.10$ & $-2.01$  &   ---    &  ---    & $132.8$ &  ---    \\ 
    \ion{Fe}{I} & $6469.21$ & $4.80$ & $-0.77$  &   ---    &  ---    &  ---    &  ---    \\ 
    \ion{Fe}{I} & $6475.63$ & $2.50$ & $-2.94$  &  $ 82.5$ &  ---    & $ 52.8$ & $ 68.5$ \\ 
%    \ion{Fe}{I} & $6494.99$ & $2.40$ & $-1.27$  &   ---    &  ---    &  ---    &  ---    \\ 
    \ion{Fe}{I} & $6546.25$ & $2.70$ & $-1.54$  &  $136.6$ &  ---    & $116.3$ &  ---    \\ 
    \ion{Fe}{I} & $6569.22$ & $4.70$ & $-0.42$  &  $ 54.3$ & $ 55.8$ & $ 42.5$ & $ 46.4$ \\ 
    \ion{Fe}{I} & $6581.21$ & $1.40$ & $-4.68$  &  $ 52.6$ & $ 63.0$ & $ 16.7$ & $ 39.1$ \\ 
%    \ion{Fe}{I} & $6591.31$ & $4.50$ & $-2.07$  &   ---    &  ---    &  ---    &  ---    \\ 
    \ion{Fe}{I} & $6593.87$ & $2.40$ & $-2.42$  &  $125.9$ &  ---    & $ 98.8$ &  ---    \\ 
    \ion{Fe}{I} & $6597.56$ & $4.80$ & $-1.07$  &  $ 21.0$ & $ 21.1$ &  ---    & $ 14.9$ \\ 
    \ion{Fe}{I} & $6608.04$ & $2.20$ & $-4.03$  &  $ 37.5$ & $ 37.9$ &  ---    &  ---    \\ 
    \ion{Fe}{I} & $6609.12$ & $2.50$ & $-2.69$  &  $ 97.6$ &  ---    & $ 64.0$ & $ 81.1$ \\ 
    \ion{Fe}{I} & $6627.54$ & $4.50$ & $-1.68$  &   ---    & $ 14.5$ &  ---    & $ 11.2$ \\ 
    \ion{Fe}{I} & $6678.00$ & $2.60$ & $-1.42$  &   ---    &  ---    & $134.5$ &  ---    \\ 
 \\ \hline \hline \\            
\end{longtable} 
\twocolumn

==> line_abundances_1column.tex <==
\onecolumn
\begin{longtable}{lccccrrrr}
\caption{Line-by-line abundances ratios in the six UVES sample stars for the odd-Z (Na and Al), alpha- (Mg, Si, Ca) $+$ Ti, iron-peak (V, Mn, Co, Cu, and Zn), and heavy-elements (Y, Zr, Ba, La, Nd, and Eu).}            
\label{tab:lines_ratios}\\   
\hline
\noalign{\smallskip}
\multirow{2}{*}{Species} & $\lambda$    & \phantom{-}\phantom{-}{ $\chi_{ex}$ }&  \multirow{2}{*}{log$gf$} &       star 1539   &    star 1363   &     star 1176  &  star 133 \\
                     &  [\AA]  &  [eV]        &                          & \multicolumn{4}{c}{[X/Fe]}\\ 
\hline\hline \endfirsthead
\multicolumn{8}{c}%
{{\bfseries \tablename\ \thetable{} -- continued}} \\ \hline
Species & $\lambda$    & \phantom{-}\phantom{-}{ $\chi_{ex}$ }&  log$gf$ &     star 1539   &    star 1363   &     star 1176  &  star 133  \\ 
\hline\hline \endhead
%                                                           1539              1363                 1176              133

\ion{Mg}{I}   &  $6318.720$  &  $5.11$  & $-2.36$  &  $+0.35$  &  $+0.47$  &  $+0.38$  &  $+0.47$ \\ 
\ion{Mg}{I}   &  $6319.242$  &  $5.11$  & $-2.80$  &  $+0.32$  &  $+0.41$  &    ---    &    ---   \\ 
\ion{Si}{I}   &  $5665.555$  &  $4.92$  & $-2.04$  &  $+0.20$  &  $+0.20$  &  $+0.25$  &  $+0.40$ \\ 
\ion{Si}{I}   &  $5666.690$  &  $5.62$  & $-1.74$  &    ---    &    ---    &  $+0.56$  &  $+0.10$ \\ 
\ion{Si}{I}   &  $5690.425$  &  $4.93$  & $-1.87$  &  $+0.35$  &  $+0.33$  &  $+0.40$  &  $+0.30$ \\ 
\ion{Si}{I}   &  $5948.545$  &  $5.08$  & $-1.30$  &  $+0.30$  &  $+0.30$  &  $+0.30$  &  $+0.35$ \\ 
\ion{Si}{I}   &  $6142.494$  &  $5.62$  & $-1.50$  &  $+0.45$  &  $+0.30$  &    ---    &  $-0.40$ \\ 
\ion{Si}{I}   &  $6145.020$  &  $5.61$  & $-1.45$  &  $+0.30$  &  $+0.50$  &  $+0.15$  &  $+0.50$ \\ 
\ion{Si}{I}   &  $6155.142$  &  $5.62$  & $-0.85$  &  $+0.25$  &  $+0.19$  &  $+0.35$  &  $+0.30$ \\ 
\ion{Si}{I}   &  $6237.328$  &  $5.61$  & $-1.01$  &  $+0.06$  &  $+0.14$  &  $+0.25$  &  $+0.35$ \\ 
\ion{Si}{I}   &  $6243.823$  &  $5.61$  & $-1.30$  &  $+0.26$  &  $+0.21$  &  $+0.35$  &  $+0.35$ \\ 
\ion{Si}{I}   &  $6414.987$  &  $5.87$  & $-1.13$  &  $+0.23$  &  $+0.06$  &  $+0.56$  &  $+0.10$ \\ 
\ion{Si}{I}   &  $6721.844$  &  $5.86$  & $-1.17$  &    ---    &    ---    &  $+0.10$  &  $+0.69$ \\ 
\ion{Ca}{I}   &  $5601.277$  &  $2.53$  & $-0.52$  &  $+0.43$  &  $+0.47$  &  $+0.09$  &  $+0.68$ \\ 
\ion{Ca}{I}   &  $5867.562$  &  $2.93$  & $-1.55$  &  $+0.26$  &  $+0.31$  &  $+0.35$  &  $+0.45$ \\ 
\ion{Ca}{I}   &  $6156.030$  &  $2.52$  & $-2.39$  &    ---    &    ---    &    ---    &    ---   \\ 
\ion{Ca}{I}   &  $6102.723$  &  $1.88$  & $-0.79$  &  $+0.60$  &  $+0.50$  &  $+0.70$  &  $+0.70$ \\ 
\ion{Ca}{I}   &  $6122.217$  &  $1.89$  & $-0.20$  &  $+0.50$  &  $+0.50$  &  $+0.70$  &  $+0.70$ \\ 
\ion{Ca}{I}   &  $6161.295$  &  $2.51$  & $-1.02$  &  $+0.36$  &  $+0.44$  &  $+0.20$  &  $+0.44$ \\ 
\ion{Ca}{I}   &  $6162.167$  &  $1.90$  & $-1.09$  &  $+0.30$  &  $+0.30$  &  $+0.70$  &  $+0.50$ \\ 
\ion{Ca}{I}   &  $6166.440$  &  $2.52$  & $-0.90$  &  $+0.15$  &  $+0.30$  &  $+0.09$  &  $+0.30$ \\ 
\ion{Ca}{I}   &  $6169.044$  &  $2.52$  & $-0.54$  &  $+0.61$  &  $+0.50$  &  $+0.05$  &  $+0.55$ \\ 
\ion{Ca}{I}   &  $6169.564$  &  $2.52$  & $-0.27$  &  $+0.65$  &  $+0.58$  &  $+0.15$  &  $+0.71$ \\ 
\ion{Ca}{I}   &  $6439.080$  &  $2.52$  & $+0.30$  &  $+0.75$  &  $+0.55$  &  $+0.70$  &  $+0.75$ \\ 
\ion{Ca}{I}   &  $6455.605$  &  $2.52$  & $-1.35$  &  $+0.30$  &  $+0.44$  &  $+0.20$  &  $+0.53$ \\ 
\ion{Ca}{I}   &  $6464.679$  &  $2.52$  & $-2.10$  &  $+0.60$  &  $+0.70$  &  $+0.55$  &  $+0.70$ \\ 
\ion{Ca}{I}   &  $6493.788$  &  $2.52$  & $-2.44$  &  $+0.50$  &  $+0.50$  &  $+0.55$  &  $+0.50$ \\ 
\ion{Ca}{I}   &  $6499.654$  &  $2.52$  & $-0.85$  &  $+0.50$  &  $+0.50$  &  $+0.10$  &  $+0.50$ \\ 
\ion{Ca}{I}   &  $6572.779$  &  $0.00$  & $-4.32$  &  $+0.60$  &  $+0.49$  &  $-0.01$  &  $+0.55$ \\ 
\ion{Ca}{I}   &  $6717.687$  &  $2.71$  & $-0.61$  &  $+0.50$  &  $+0.50$  &  $+0.25$  &  $+0.50$ \\ 
\ion{Ti}{I}   &  $5922.108$  &  $1.05$  & $-1.46$  &  $+0.51$  &  $+0.55$  &  $+0.18$  &  $+0.48$ \\ 
\ion{Ti}{I}   &  $5941.750$  &  $1.05$  & $-1.50$  &  $+0.36$  &  $+0.40$  &  $+0.28$  &  $+0.33$ \\ 
\ion{Ti}{I}   &  $5965.825$  &  $1.88$  & $-0.42$  &  $+0.30$  &  $+0.45$  &  $+0.08$  &  $+0.34$ \\ 
\ion{Ti}{I}   &  $5978.539$  &  $1.87$  & $-0.53$  &  $+0.40$  &  $+0.30$  &  $+0.13$  &  $+0.37$ \\ 
\ion{Ti}{I}   &  $6064.623$  &  $1.05$  & $-1.94$  &  $+0.31$  &  $+0.30$  &  $+0.05$  &  $+0.28$ \\ 
\ion{Ti}{I}   &  $6091.169$  &  $2.27$  & $-0.42$  &  $+0.14$  &  $+0.26$  &    ---    &  $+0.23$ \\ 
\ion{Ti}{I}   &  $6126.214$  &  $1.07$  & $-1.43$  &  $+0.30$  &  $+0.40$  &  $+0.10$  &  $+0.30$ \\ 
\ion{Ti}{I}   &  $6258.110$  &  $1.44$  & $-0.36$  &  $+0.10$  &  $+0.15$  &  $+0.19$  &  $+0.10$ \\ 
\ion{Ti}{I}   &  $6261.106$  &  $1.43$  & $-0.48$  &  $+0.30$  &  $+0.50$  &  $+0.10$  &  $+0.30$ \\ 
\ion{Ti}{I}   &  $6312.240$  &  $1.46$  & $-1.60$  &  $+0.24$  &  $+0.40$  &  $+0.09$  &  $+0.35$ \\ 
\ion{Ti}{I}   &  $6336.113$  &  $1.44$  & $-1.74$  &  $+0.20$  &  $+0.34$  &  $+0.26$  &  $+0.18$ \\ 
\ion{Ti}{I}   &  $6554.238$  &  $1.44$  & $-1.22$  &  $+0.10$  &  $+0.15$  &  $+0.06$  &  $+0.26$ \\ 
\ion{Ti}{I}   &  $6556.077$  &  $1.46$  & $-1.07$  &  $+0.30$  &  $+0.40$  &  $+0.22$  &  $+0.32$ \\ 
\ion{Ti}{I}   &  $6599.113$  &  $0.90$  & $-2.09$  &  $+0.28$  &  $+0.30$  &  $+0.10$  &  $+0.30$ \\ 
\ion{Ti}{I}   &  $6743.127$  &  $0.90$  & $-1.73$  &  $+0.20$  &  $+0.26$  &  $-0.19$  &  $+0.20$ \\ 
\ion{Ti}{II}  &  $5418.751$  &  $1.58$  & $-2.13$  &  $+0.30$  &  $+0.38$  &  $+0.30$  &  $+0.43$ \\ 
\ion{Ti}{II}  &  $6491.580$  &  $2.06$  & $-2.10$  &  $+0.30$  &  $+0.38$  &  $+0.30$  &  $+0.43$ \\ 
\ion{Ti}{II}  &  $6559.576$  &  $2.05$  & $-2.35$  &  $+0.26$  &  $+0.30$  &  $+0.23$  &  $+0.36$ \\ 
\ion{Ti}{II}  &  $6606.970$  &  $2.06$  & $-2.85$  &  $+0.35$  &  $+0.30$  &  $+0.31$  &  $+0.30$ \\ 
\hline
\ion{Na}{I}   &  $5682.633$  &  $2.10$  & $-0.71$  &  $-0.32$  &  $-0.30$  &  $-0.00$  &  $+0.31$ \\ 
\ion{Na}{I}   &  $5688.194$  &  $2.10$  & $-1.40$  &  $-0.35$  &  $-0.30$  &  $-0.30$  &  $+0.20$ \\ 
\ion{Na}{I}   &  $6154.230$  &  $2.10$  & $-1.56$  &  $-0.15$  &  $-0.00$  &    ---    &  $+0.30$ \\ 
\ion{Na}{I}   &  $6160.753$  &  $2.10$  & $-1.26$  &  $-0.35$  &  $-0.00$  &  $-0.35$  &  $+0.00$ \\ 
\ion{Al}{I}   &  $6696.185$  &  $4.02$  & $-1.58$  &  $-0.30$  &  $-0.30$  &  $<+0.30$  &  $<+0.30$ \\ 
\ion{Al}{I}   &  $6698.673$  &  $3.14$  & $-1.65$  &  $-0.29$  &  $+0.00$  &  $<+0.30$  &  $<+0.30$ \\ 
\hline
\ion{V}{I}    &  $5703.560$  &  $1.05$  & $-0.21$  &  $+0.05$  &  $+0.17$  &    ---    &  $+0.14$ \\ 
\ion{V}{I}    &  $6081.440$  &  $1.05$  & $-0.58$  &  $-0.02$  &  $+0.17$  &    ---    &  $+0.02$ \\ 
\ion{V}{I}    &  $6090.220$  &  $1.08$  & $-0.16$  &  $+0.05$  &  $+0.14$  &  $-0.32$  &  $+0.08$ \\ 
\ion{V}{I}    &  $6119.520$  &  $1.06$  & $-0.47$  &  $-0.05$  &  $+0.08$  &  $-0.26$  &  $-0.05$ \\ 
\ion{V}{I}    &  $6199.190$  &  $0.29$  & $-1.48$  &  $+0.05$  &  $+0.17$  &    ---    &  $-0.11$ \\ 
\ion{V}{I}    &  $6243.100$  &  $0.30$  & $-0.88$  &  $+0.11$  &  $+0.38$  &    ---    &  $+0.05$ \\ 
\ion{V}{I}    &  $6251.820$  &  $0.29$  & $-1.44$  &  $+0.11$  &  $+0.32$  &  $-0.41$  &  $-0.05$ \\ 
\ion{V}{I}    &  $6274.650$  &  $0.27$  & $-1.72$  &  $-0.05$  &  $+0.11$  &    ---    &  $-0.08$ \\ 
\ion{Mn}{I}   &  $5394.669$  &  $0.00$  & $-3.55$  &  $-0.40$  &  $-0.50$  &  $-0.40$  &  $-0.50$ \\ 
\ion{Mn}{I}   &  $6013.513$  &  $3.07$  & $-0.40$  &  $-0.30$  &  $-0.25$  &  $-0.30$  &  $-0.30$ \\ 
\ion{Mn}{I}   &  $6016.640$  &  $3.07$  & $-0.22$  &  $-0.35$  &  $-0.50$  &  $-0.60$  &  $-0.40$ \\ 
\ion{Mn}{I}   &  $6021.800$  &  $3.08$  & $-0.10$  &  $-0.30$  &  $-0.45$  &  $-0.25$  &  $-0.50$ \\ 
\ion{Co}{I}   &  $5212.691$  &  $3.51$  & $-0.11$  &    ---    &  $+0.15$  &    ---    &  $+0.15$ \\ 
\ion{Co}{I}   &  $5301.047$  &  $1.71$  & $-2.00$  &  $+0.00$  &  $+0.10$  &    ---    &  $+0.10$ \\ 
\ion{Co}{I}   &  $5342.708$  &  $4.02$  & $+0.69$  &  $+0.05$  &  $+0.05$  &    ---    &  $+0.00$ \\ 
\ion{Co}{I}   &  $5454.572$  &  $4.07$  & $+0.24$  &    ---    &  $+0.10$  &  $+0.20$  &  $+0.10$ \\ 
\ion{Co}{I}   &  $5647.234$  &  $2.28$  & $-1.56$  &  $+0.05$  &  $+0.05$  &  $+0.00$  &  $+0.30$ \\ 
\ion{Co}{I}   &  $6188.996$  &  $1.71$  & $-2.45$  &  $+0.00$  &  $+0.00$  &  $+0.00$  &  $+0.30$ \\ 
\ion{Cu}{I}   &  $5105.537$  &  $1.39$  & $-1.52$  &  $-0.40$  &  $-0.15$  &  $-0.30$  &  $-0.35$ \\ 
\ion{Cu}{I}   &  $5218.197$  &  $3.82$  & $+0.00$  &  $-0.30$  &  $+0.00$  &  $+0.05$  &  $+0.00$ \\ 
\ion{Zn}{I}   &  $6362.339$  &  $5.79$  & $-0.30$  &  $-0.30$  &  $-0.20$  &  $+0.30$  &  $-0.10$ \\ 
\hline
\ion{Y}{I}    &  $6435.004$  &  $0.07$  & $-0.82$  &  $-0.30$  &  $-0.32$  &  $-0.30$  &  $+0.00$ \\ 
\ion{Y}{II}   &  $6795.414$  &  $1.74$  & $-1.19$  &  $+0.20$  &  $+0.00$  &  $+0.00$  &    ---   \\ 
\ion{Zr}{I}   &  $6127.475$  &  $0.15$  & $-1.06$  &  $-0.08$  &  $+0.05$  &    ---    &  $-0.08$ \\ 
\ion{Zr}{I}   &  $6134.585$  &  $0.00$  & $-1.42$  &  $+0.05$  &  $+0.20$  &    ---    &  $+0.23$ \\ 
\ion{Zr}{I}   &  $6140.535$  &  $0.52$  & $-1.60$  &    ---    &    ---    &    ---    &  $-0.50$ \\ 
\ion{Zr}{I}   &  $6143.252$  &  $0.07$  & $-1.10$  &  $-0.14$  &  $+0.02$  &    ---    &  $-0.08$ \\ 
\ion{Ba}{II}  &  $5853.675$  &  $0.60$  & $-1.10$  &  $+0.92$  &  $+1.00$  &  $+1.00$  &  $+1.05$ \\ 
\ion{Ba}{II}  &  $6141.713$  &  $0.70$  & $-0.08$  &  $+0.60$  &  $+0.80$  &  $+0.65$  &  $+0.80$ \\ 
\ion{Ba}{II}  &  $6496.897$  &  $0.60$  & $-0.32$  &  $+1.00$  &  $+1.00$  &  $+1.10$  &  $+1.20$ \\ 
\ion{La}{II}  &  $6262.287$  &  $0.40$  & $-1.60$  &  $+0.00$  &  $+0.00$  &  $+0.17$  &  $+0.26$ \\ 
\ion{La}{II}  &  $6320.376$  &  $0.17$  & $-1.56$  &  $+0.00$  &  $+0.00$  &  $+0.14$  &  $+0.30$ \\ 
\ion{La}{II}  &  $6390.477$  &  $0.32$  & $-1.41$  &  $+0.25$  &  $+0.17$  &  $+0.00$  &  $+0.26$ \\ 
\ion{Nd}{II}  &  $6740.078$  &  $0.06$  & $-1.53$  &  $+0.45$  &  $+0.15$  &  $+0.17$  &  $-0.30$ \\ 
\ion{Nd}{II}  &  $6790.372$  &  $0.18$  & $-1.77$  &  $+0.55$  &  $+0.40$  &  $+0.00$  &  $-0.30$ \\ 
\ion{Nd}{II}  &  $6549.525$  &  $0.06$  & $-2.01$  &  $+0.40$  &  $+0.30$  &  $+0.00$  &    ---   \\ 
\ion{Eu}{II}  &  $6437.640$  &  $1.32$  & $-0.32$  &  $+0.55$  &  $+0.55$  &  $+0.65$  &  $+0.50$ \\ 
\ion{Eu}{II}  &  $6645.064$  &  $1.38$  & $+0.12$  &  $+0.50$  &  $+0.55$  &  $+0.50$  &  $+0.70$ \\ 
\\ \hline \hline \\            
\end{longtable} 
